Revisiting flares in Sagittarius A* based on general relativistic magnetohydrodynamic numerical simulations of black hole accretion

High-resolution observations with GRAVITY-VLTI instrument have provided abundant information about the flares in Sgr A*, the supermassive black hole in our Galactic center, including the time-dependent location of the centroid (a "hot spot"), the light curve, and polarization. Yuan et al. (2009) proposed a "coronal mass ejection" model to explain the flares and their association with the plasma ejection. The key idea is that magnetic reconnection in the accretion flow produces the flares and results in the formation and ejection of flux ropes. The dynamical process proposed in the model has been confirmed by three-dimensional GRMHD simulations in a later work. Based on this scenario, in our previous works the radiation of the flux rope has been calculated analytically and compared to the observations. In the present paper, we develop the model by directly using numerical simulation data to interpret observations. We first identify flux ropes formed due to reconnection from the data. By assuming that electrons are accelerated in the reconnection current sheet and flow into the flux rope and emit their radiation there, we have calculated the time-dependent energy distribution of electrons after phenomenologically considering their injection due to reconnection acceleration, radiative and adiabatic cooling. The radiation of these electrons is calculated using the ray-tracing approach. The trajectory of the hot spot, the radiation light curve during the flare, and the polarization are calculated. These results are compared with the GRAVITY observations and good consistencies are found.

==> reply.tex <==
1. Referee report: 

Page 2 C2L3: super-keplerian motion of flux ropes -> The authors cite Lin et al. 2023, who cites Cemeljic et al. 2022. I fail to see the reasoning behind super-Keplerianity since Cemeljic et al. explicitly says that MADs and SANEs have sub-Keplerian velocity. I understand that the jet-wind boundary is unstable to tearing modes, and that produces the largest plasmoids, which look like they are radially ejected out. Since the authors are the same as Lin et al 2023, I ask for a clarification. 

Response:

Lin et al. 2023 is an analytical work. In that work, the super-Kelerian motion of the ejected flux rope is realized by assuming that the field line connecting the flux rope to the underlying accretion flow is rigidly rotating so the flux rope has the same angular velocity with the foot point of the field line. In the present work, however, by checking carefully the simulation data, we do not find obvious super-Keplerian motion of the flux rope but its velocity is close to the Kepler-velocity when it is not too far away from the black hole (lower panel of Figure 8). On the other hand,  as we describe in Section 4.1, the apparent super-Keplerian is now attributed to its radial motion along the line of sight. We have modified the presentations to clarify. 

In addition, we would like to clarify that different from some other works, the flux ropes in our model are not formed within the current sheet due to the tearing mode instability (Figure 1). The later one, we think, make minor contribution to the radiation compared to the flux rope. Rather, the formation of the flux rope in our model is due to the closed field line formed by reconnection, as we have described in detail in Yuan et al. (2009) and in Cemeljic et al. (2022).  We have clarified this point in  Page 2 in this revised version.


2. Referee report: 

Page 2 C2L15: please cite a reference for the periodicity of flux rope ejections. Does the periodicity depend on the initial magnetic field? I see that Cemeljic et al 2022 is cited in section 4.4. Please also add the citation here. Also is this periodicity applicable for both MAD and SANE flows? 

Response: 

The citation is Cemeljic et al 2022 and we have added it 
. They found the periodicity does not depend on the initial magnetic field and the period of ~1000r_g/c is applicable for both MAD and SANE flows. You can refer to Section 3.3 in their paper for detail. But here we cite some of their statements for convenience. A screenshot is provided in the Appendix.

"This implies a period of ∼1000rg/c. Such a period matches the orbiting timescale of both SANE and MAD at 20–30rg well, which is slightly larger than the Keplerian timescale, since the angular velocities of both SANE and MAD are sub-Keplerian (Yuan & Narayan 2014). "

"This scenario is enhanced by the fact that there seems to be no difference in terms of the periodicity of the formation of the flux ropes in the SANE and MAD cases, although MAD is much less turbulent compared to SANE."

3. referee: Grid resolution: please mention more details about the SMR in the grid: what is the base grid resolution, the number of refinement levels and the refinement criteria? It is important as the authors track the evolution of a flux rope over time, and rapid decrease in resolution can cause extra dissipation. For example, the jet and wind region in Figure 9 look quite pixelated. 

4.reply: We have added two tables (Table 1 & Table 2) and some descriptions to the SMR. For a refinement region, each additional level means that the grid of this area is refined by a factor of 2 for all directions based on the previous level grid. In the jet and wind region, the grid is at least 2-level refined in all direction. We believe the resolution is adequate to track the evolution of a flux rope.

The supplementary description is provided in Page 3 C2L20 
 
4. Page 4 C1L51: Bp/Bphi in the jet depends on the jet cylindrical radius (as can be seen in Fig 4): the outer part of the jet becomes increasingly toroidal field dominant, and hence is susceptible to current-driven instabilities.

5. Page 5 C2L19: the flux rope moves more straightly in the r direction -> perhaps “moves primarily in the radial direction”?

reply: here we want to stress the movement of the flux rope in the radial direction is much more straight in the MAD cases than in the SANE cases.

We have changed an alternative expression in Page 7 C1L2.

6. Page 5 C2L36: “Note that in the 3D simulations, the flux rope does not appear as a spherical blob as in the 2D cases” -> In 2D, the blobs are actually thick rings as there is azimuthal symmetry enforced. In 3D, I expect the flux ropes would be deformed spherical structures due to azimuthal shearing.

reply: Thank for the correction. The shape of the blobs in 2D should be thick rings. In 3D, the flux ropes are actually not spherical but elongated in the azimuthal direction like ropes as is indicated by the name. The configuration of a single magnetic field line of the flux rope is like a bent and twisted spring. And usually these spring-like flux ropes are tangled and twined each other to form a concrete structure like a braid. And as you suggest, the structures would further be deformed under shearing, which is however, not considered in our work. Maybe in the future work we would reconsider this by involving different parts of the fluid elements enveloped in the flux rope rather than simply regard them as a unity.

We have modified the corresponding argument in Page 7 C1L20

7.Referee: Figure 6: It looks like it takes ~100 rg/c for the flux rope to travel ~20 rg in height. Assuming that there is some azimuthal motion as well, what is the Lorentz factor of this flux rope? Is it even relativistic? How do the authors distinguish between eddy features brought about by turbulence and flux ropes?

Reply: In Figure 6, the slice plots are actually not made at a same phi. Instead we pick the one where the structure of the current sheet and flux rope is most obvious from several adjacent phi-slice plots at each time step. Because the position of the flux rope can have noticeable difference even for the two successive phi-slice plots. Therefore we consider it is very inaccurate to identify its location just by the plots (and that is why we choose to integrate the fluid velocity over time to trace the flux rope). The criteria we distinguish eddies and flux rope is to check whether it has a time lasting current sheet structure at the stage it is newly formed (as in Figure 6). Besides, the accretion flow of MADs are less turbulent and the interference of eddies is very minor compared to the SANE cases. 

8. referee: Page 7 C1L28: saperatix -> separatrix.
reply: corrected

9. referee Page 7 C2L25: “in the high accretion rate state and low accretion rate state” -> do the authors mean the magnetic flux eruption phases in MADs here? Or the relatively higher accretion rate in the MAD simulations during 5000-15000rg/c compared to the “low” accretion rate during 20000-40000rg/c? The latter usually occurs when the torus has lost a significant amount of gas through the outer radial boundary. Is that what happens in these simulations? What is the outer radius of the grid?

reply: Sorry for the ambiguous statements. The former one is what we want to express. We have rewritten the sentence (Page 7 C2L27) to make it clearer.

10. Referee: Figure 8: are the radial and angular velocities defined with contra variant or covariant 4-velocities? There seems to be a typo in the plot according to Eqn 8. Does the trajectory calculation via eqn 8 line up with the actual flux rope trajectory since the authors know both the flux rope location as well as the fluid velocity within it independently from the GRMHD data? Could the authors clarify if they are recalculating the flux rope velocity according to its location or the other way around?

reply: Thanks for pointing out the typo. We actually adopt contra-variant velocities when making these plots. We have corrected the typo in Figure 8. As we have mentioned before, the flux rope location is very hard to identify precisely merely based on the phi-slice plots, since at most time the flux rope structure can appear at a wide range of phi. And the position of the flux rope in these phi-slice plots can vary a lot. Therefore we choose a different approach: we first find a flux rope that is newly born. And at this phase the flux rope mostly only appear in one or two phi-slices. Then we identify the flux rope center in a phi-slice and integrate the velocity provided by the simulation to get its subsequent location. Once we know its new location, we can obtain its velocity once again from the simulation data repeatably.

11. referee: Table 2: how does the blob parameters tie in with the flux rope characteristics from the GRMHD simulation? Also, the authors could include the unit of the accretion rate here (Msun/yr) as they have done for the other quantities.

The GRMHD simulation only provide gas density, gas pressure, and magnetic field etc. The parameters in Table 4 now mainly determine the emitting electron distribution, especially the time-dependent non-thermal electrons. For example, we could determine the temperature of thermal electrons by two parameters R_high and R_low combined with the plasma beta acquired from the simulation data according to Eq 15. The unit of accretion rate has been added as suggested.


12. Page 10 Eqn 17: could the authors point out where in Cemeljic et al 2022 is it mentioned that the current sheet layer is 100 degrees wide in azimuth? Perhaps in a figure?

reply: You can refer to the last sentence in the label of Figure 2 on page 3. What they mention there is the flux rope. Because the flux rope is the product of reconnection and it is formed on the top tip of the current layer (Figure 1), it is reasonable to regard them have a similar extension in azimuth. A screenshot is provided in the appendix for convenience. 


13. Referee: Eqn 17: in the reconnection zone, wouldn’t B_0 be very small?

reply: In the reconnection zone, B is indeed very small. However here B0 is not the field strength in the reconnection current layer but instead in the reconnection inflow region, which is chosen 1 r_g perpendicularly away from the current layer. And in this area, B_0 is not small so that enough injection energy could be provided.


14. Page 10 C1L12: “cite” -> site
reply: corrected

15. Page 10 C1L29: how does the flux rope have a large magnetic field if there’s reconnection? 

reply: We have to stress again the flux rope is not the plasmoid formed in the current sheet. Although in some literature, these two terms are used interchangeable. In our work magnetic flux rope is field topology characterized by bundles of helical magnetic field lines collectively spiraling around a common axis, and one of its essential properties is the enhanced magnetic field strength. 


16. Page 10 C1L50: cooing -> cooling
corrected

17. Page 10 C2L16: the authors could draw a circle with the expanding radius and check whether the expansion rate is roughly correct or not. The assumption is that the blob or plasmoid follows the motion of the center of the flux rope, which the authors are already tracking.

reply: Sorry to make some explanations that we do not add the plot. The expansion rate is for the non-thermal electrons not the magnetic field lines. The actual electrons' space distribution, however, is indistinguishable in our work. Even if they have a same expansion rate, it is still non-trivial to measure how fast the flux rope expands unless we can trace a single magnetic field line over time. The stream plot is made by sampling magnetic field vectors and integrate them to form lines. The appearing size of the flux rope field lines is determined by how you make the plot. For example if we increase the sampling number of the stream lines, there will be more "circle loops" for the flux rope and the most central loop will become smaller. Therefore, we suggest that the field line plots should only be an instructive illustration rather than a quantitatively-analyzing object. The expansion rate is adopted from Dodds-Eden2010 and it also satisfies the restriction given by the GRAVITY collaborations.


18. Does the injection of power from the magnetic reconnection only occur at/near the X-point? Is there continuous injection? Or is there a one-time injection of accelerated electrons in the blob, which is then allowed to evolve and cool? What is the magnetic field direction chosen for the spherical blob?

When calculating the injection power, we consider the whole area of the current layer. The actually injection position is not specified in this work because we only care about the total injection power and the spectrum of the non-thermal electrons. In practical situation, the energy is dissipated most strongly near the magnetic null which appears as an X-or Y-point in the 2D plots. The injection is continuous and the injection power is estimated according to Equation 17. When doing the radiative transfer calculation, the magnetic field direction can be determined directly from the GRMHD simulation data since we have already known the blob's position.

19. Table 3: Please provide references for the mass and distance of Sgr A* used in the raytracing. The authors quote different values for M and D in their introduction.

The mass is from GRAVITY2018 (A&A, 618, L10) and the distance is from GRAVITY2019 (A&A, 625, L10).

20. Page 11 C1L42: “The observer is up above the black hole (penetrated by the spin axis)” -> perhaps “The observer is located above the black hole, i.e., at an inclination of 90 degrees.”?

Sorry for the ambiguous statement. The observer is located above the black hole and the inclination angle is 0 degree to the spin axis. We have rewritten the paragraph in Section 4.1 to make it clearer.

21. Page 11 C2L25: it seems to me that there are several free parameters in the blob model: BH mass, distance, inclination, blob power-law parameters such as power-law index, efficiency, etc. are all chosen. Additionally, the authors are not modeling the actual physics of the flux rope, but instead there are modeling a spherical blob, ignoring the effects of shearing. For what I gather, they choose to use the evolving location of the flux rope and the magnitude of the magnetic field and the gas temperature contained within. The authors should make it clear which quantities are taken directly from the GRMHD simulation, and which ones are assumed, perhaps such that the light curve profile from the raytracing matches the observed NIR lightcurve or the centroid behavior roughly matches the observations.

reply: q1: yes. q2: yes. q3: yes. 

The flux rope location is totally determined by the simulation. And the centroid trajectory (if neglecting the modification of radiation) can also be determined. The light curve and polarization are heavily dependent on some other parameters, particularly that influence the distribution of the non-thermal electrons. BH mass and distance can be well restricted by observations (especially from EHT and GRAVITY collaborations). Magnetic field and ion temperature can be directly obtained from the simulation, but the concrete values can only be specified when the accretion rate and black hole mass is given for the simulation is dimensionless. Thermal electron temperature is derived by a model and extra parameters are needed. Injection energy can be obtained from the simulation but lots of simplifications have to be made to achieve this. To determine the injected non-thermal electrons, acceleration efficiency, power law index and higher energy cut-off (which although is not so important) should additionally be assumed. Finally, because we take into consideration of further cooling effects, some parameters associated with cooling, i.e., expansion rate is needed. And because we neglect the shearing effect and simplify the shape of the flux rope, the length-scale should also be estimated for the further radiation calculation.  
